Modeling Global and Local Node Contexts for Text Generation from Knowledge Graphs

Recent graph-to-text models generate text from graph-based data using either global or local aggregation to learn node representations. Global node encoding allows explicit communication between two distant nodes, thereby neglecting graph topology as all nodes are directly connected. In contrast, local node encoding considers the relations between neighbor nodes capturing the graph structure, but it can fail to capture long-range relations. In this work, we gather both encoding strategies, proposing novel neural models which encode an input graph combining both global and local node contexts, in order to learn better contextualized node embeddings. In our experiments, we demonstrate that our approaches lead to significant improvements on two graph-to-text datasets achieving BLEU scores of 18.01 on AGENDA dataset, and 63.69 on the WebNLG dataset for seen categories, outperforming state-of-the-art models by 3.7 and 3.1 points, respectively.

==> 3_1-Transformers.tex <==
\subsection{Self-Attention Networks (SAN)}
\label{sec:transformers}
Transformers \cite{NIPS2017_7181} employ self-attention networks (SAN) for implementing both the encoder and the decoder, enabling efficient and paralleled computation by leveraging a self-attention mechanism for global context modeling.

% SANs produce representations by applying attention mechanisms to each pair of tokens from a input sequence $X = \{ x_1, ..., x_n \}$, regardless of their distance, computing a new sequence $Z = \{ z_1, ..., z_n \}$:

In a different perspective of SANs, we can treat the attention as edges in a complete graph (see Figure \ref{fig:kg}b) and adopt message passing on those artificial edges to learn node representations. In particular, we compute the \textit{global convolution} for a node $v \in \mathcal{V^{'}}$, adopting $\textrm{AGGR}^{(l)}(.)$ as:
\begin{equation}
h_{\mathcal{N}(v)}^{(l)} = \sum_{u \in \mathcal{V}} \alpha_{vu} \big( u \, W^{(l)}_{v} \big)
\end{equation}

% \begin{equation}
% z_i = \sum_{j=1}^{n} \alpha_{ij} \big( x_j \, W^{V} \big) \label{eq:1}
% \end{equation}
where $W^{(l)}_{v} \in \mathbb{R}^{d_x \times d_z}$ is a parameter. The attention weight $\alpha_{ij}$ of each node $v_i$ is calculated as:
$$
\alpha_{ij} = \frac{\exp(e_{ij})}{ \sum_{k=1}^n \exp(e_{ik})}
$$
where:
$$
e_{ij} = \frac{ \big( v_i W^{(l)}_{q} \big)  \big( v_j W^{(l)}_{k} \big) }{\sqrt{d_z}}
$$
is a attention function which measures how well the nodes $v_i$ and $v_j$ match. $W^{(l)}_{q}, W^{(l)}_{k} \in \mathbb{R}^{d_x \times d_z}$ are model parameters.

% where the vectors $\alpha_{i} = (\alpha_{i1}, ..., \alpha_{in})$ capture the correspondences between $v$ and other nodes. After compute the equation~\ref{eq:2}, we have the node representation $g^{'}_{v} \in \mathcal{V^{'}}$.

% In addition, the performance of SANs are improved by multi-head attention. The multi-head attention consists of $h$ attention heads, and each of them learns a distinct attention function. 



Finally, the outputs $Z = \{ z_1, ..., z_n \}$ of all attention heads are concatenated and projected to the original dimension of $x$, followed by feed-forward layers, residual connection, and layer normalization:
\begin{equation}
\begin{aligned}
   \Tilde{z}_i &= \text{LayerNorm}(x_i + \text{LayerNorm}(z_i)) \\
z^{'}_{i} &= \text{FFN}(\Tilde{z}_i) \,\, .
\end{aligned}
\label{eq:2}
\end{equation}

%\footnote{Please, refer to \citet{NIPS2017_7181} for more details.}.

%In section~\ref{sec:model}, we demonstrate how we leverage SANs, employing them as a complete graph.

==> 3_2-GNN.tex <==


%In the following section, we explain ours choices, proposing an relational multi-attention GNN approach.


==> tmp <==


While knowledge graphs Knowledge graphs (KG) are important structured
repositories that describe world knowledge as relationships between
entities and are useful for numerous applications, they are often
difficult for human beings to use and understand. With the emergence
of the semantic web, the rapid increase of Linked data and the
proliferation of knowledge bases, there is a growing need for
technologies that give humans easy access to knowledge graphs and
more generally, to the machine-oriented Web of data. Because it maps
data to text, Natural Language Generation (NLG) provides a natural
mean for presenting this data in an organized, coherent and accessible
way. It can be used to display the content of linked data or of
knowledge bases to lay users; to generate explanations, descriptions
and summaries from DBPedia or from knowledge bases; to guide the user
in formulating knowledge base queries.



with the emergence of the ``Big Data'' phen
With
As shown in \cite{rector2004owl}, the basic standards (e.g., RDF, OWL)
established by the Semantic Web community for representing data and
ontologies are difficult for human beings to use and understand. With
the development of the semantic web, the rapid increase of Linked
Data, the proliferation of  knowledge bases and more generally,
with the emergence of the ``Big Data'' phenomenon, there is
consequently a growing need in the semantic web (SW) community for
technologies that give humans easy access to the machine-oriented Web
of data.

Because it maps data to text, Natural Language Generation (NLG)
provides a natural mean for presenting this data in an organized,
coherent and accessible way. It can be used to display the content of
linked data or of knowledge bases to lay users; to generate
explanations, descriptions and summaries from DBPedia or from
knowledge bases; to guide the user in formulating knowledge base
